Approaches to human activity recognition via passive radar

The thesis explores novel methods for Human Activity Recognition (HAR) using passive radar with a focus on non-intrusive Wi-Fi Channel State Information (CSI) data. Traditional HAR approaches often use invasive sensors like cameras or wearables, raising privacy issues. This study leverages the non-intrusive nature of CSI, using Spiking Neural Networks (SNN) to interpret signal variations caused by human movements. These networks, integrated with symbolic reasoning frameworks such as DeepProbLog, enhance the adaptability and interpretability of HAR systems. SNNs offer reduced power consumption, ideal for privacy-sensitive applications. Experimental results demonstrate SNN-based neurosymbolic models achieve high accuracy making them a promising alternative for HAR across various domains.

==> sections/acknowledgements.tex <==
\selectlanguage{italian}
\chapter*{Ringraziamenti}
Desidero esprimere la mia profonda gratitudine al Professor Federico Cerutti, mio relatore, per avermi dato l’opportunità di lavorare a questo progetto e per il suo prezioso sostegno e guida durante l’intero percorso della tesi.
Un ringraziamento speciale va al Dottor Marco Cominelli, mio correlatore, per i suoi consigli sempre puntuali e per l'aiuto fondamentale che ha contribuito alla realizzazione di questo lavoro.

Rivolgo un sincero ringraziamento ai miei genitori e a mia sorella, che con il loro affetto, pazienza e sostegno costante mi hanno accompagnato lungo il mio intero percorso accademico. Un pensiero speciale va anche ai miei amici, che con la loro presenza, incoraggiamento e i momenti di spensieratezza mi hanno aiutato a mantenere la giusta motivazione e serenità per raggiungere questo traguardo.
